Estimating Sparse Discrete Distributions Under Local Privacy and Communication Constraints

We consider the problem of estimating sparse discrete distributions under local differential privacy (LDP) and communication constraints. We characterize the sample complexity for sparse estimation under LDP constraints up to a constant factor and the sample complexity under communication constraints up to a logarithmic factor. Our upper bounds under LDP are based on the Hadamard Response, a private coin scheme that requires only one bit of communication per user. Under communication constraints, we propose public coin schemes based on random hashing functions. Our tight lower bounds are based on the recently proposed method of chi squared contractions.

==> rappor-sparse.tex <==
\section{An Upper Bound from RAPPOR}

\begin{algorithm2e}[ht]
\DontPrintSemicolon
\SetAlgoLined
{\bf Input: }{$2\nse$ samples from unknown $s$-sparse $\p$.}
Apply RAPPOR to the samples.\;
Keep the $3s$ symbols from the first $N_1$ samples with highest $M_i$'s.\;
Apply RAPPOR to estimate only the distributions over these $3s$ elements over the next $N_1$ samples. 
\caption{Sparse estimation using RAPPOR}
\end{algorithm2e}


We will use the following two sided tail bound (McDiarmid's inequality. 
\begin{lemma}
Let $Y_1, \ldots, Y_n$ be independent random variables with $Y_i\in[-1,1]$, and $Y = Y_1+\dots+Y_\ns$, and $\mu= \expectation{Y}$. Then for $\delta>0$, 
\begin{align}
\Prb\Paren{\absv{Y-\mu}>t} \le 2\exp\Paren{-{t^2}/{2n}}\nonumber.
\end{align}
\end{lemma}

Consider the first $\nse$ messages obtained by applying RAPPOR. Let $\ms_i$ be the number of one's in the $i$th location of the messages. 


Then, $\EE[M_i]=\nse (\p(i) \gamma+\beta)$, where $\beta=1/(e^\eps+1)$, and $\gamma=(e^\eps-1)/(e^\eps+1)$. 

Let $S$ be the set of elements with non zero probability. If $i\in [k]\setminus S$, then $p(i)=0$. Hence,
\lnote{switched $k$ and $s$ in the fractions}
\[
\Prb\Paren{M_i\ge \nse\beta +C_1\sqrt{\nse \log \frac ks}}\le \Paren{\frac sk}^{C_1^2/2}.
\]
Therefore, by Markov's inequality
\begin{align}
\Prb\Paren{|i\in [k]\setminus S: M_i\ge \nse\beta +C_1\sqrt{\nse \log \frac ks}|>s}\le \Paren{\frac sk}^{C_1^2/2-1}.
\end{align}
We condition on the event $E$ that at most $s$ symbols in $[k]\setminus S$ appear more than $M^\ast\colon=\nse\beta +C_1\sqrt{\nse \log \frac ks}$ times. Therefore, a symbol $i$ is not selected after the first stage only if it appears at most  $M^\ast$ times. 

Let $T$ be the set of symbols selected after the first round. We claim that $\EE\left[\Prb(T^c)\right]<\alpha/10$. 
\begin{align}
\EE\left[\Prb(T^c)\right|E] \le 
\sum_i\p(i)\Prb\Paren{M_i \le M^\ast}
\le \sum_{i:\p(i)>\alpha/20s}\p(i)\Prb\Paren{M_i<M^\ast}
+\frac{\alpha}{20},
\end{align}
Now note that 
\begin{align}
\EE\left[M_i-M^\ast\right]=\nse \gamma\p(i)-C_1\sqrt{\nse \log \frac ks},
\end{align}
and for $\nse = 10000 C_1^2 \frac{s^2\log \frac ks}{\alpha^2\gamma^2}$, using $\p(i)>\alpha/20s$,
\begin{align}
\frac12 \nse \gamma\p(i)-C_1\sqrt{\nse \log \frac ks}\ge 0
\end{align}
giving
\begin{align}
\EE\left[M_i-M^\ast\right]\ge\frac 12\nse \gamma\p(i).
\end{align}
Applying McDiarmid's inequality again, 
\begin{align}
\Prb\Paren{M_i \le M^\ast} 
&= \Prb\Paren{M_i \le \EE[M_i] -(\EE[M_i] -M^\ast)}\\
&\le \exp\Paren{-\frac{\nse\gamma^2\p(i)^2}{8}}
\end{align}

Now for $\p(i)=(1+\zeta_i)\alpha/20s$ where $\zeta_i>0$, we have 
\begin{align}
\nse \p(i)^2\gamma^2= 25 C_1^2(1+\zeta_i)^2 \log \frac ks,
\end{align}
and therefore, 
\begin{align}
\EE\left[\Prb(T^c)\right|E] \le 
\frac \alpha{20s}\sum_i (1+\zeta_i)\exp\Paren{-25C_1^2 (1+\zeta_i)^2\log \frac ks}\le \frac {\alpha}{20}.
\end{align}








\snote{The maths seems correct to me. But I don't see how the factor $\log(k/s)$ is used here. So I am a bit skeptical.}

\lnote{Do we need to keep the following lines? Does not seem related to the previous part.}

Then for $\p(i)>\alpha/4s$,   
\begin{align}
\nse \gamma^2 \p(i)^2 > C/16\cdot \log (k/s). 
\end{align}

Therefore, 
\begin{align}
\Prb\Paren{{M_j-M_i}\ge0} \le \exp\Paren{-\frac{C}{16}\log \frac ks} = \Paren{\frac ks}^{C/4}.
\end{align}

\anote{From here $s<d^{0.99}$ is straight forward. For larger $s$, all we need to do is to rewrite the thing above in terms of $p_i$ and bound the total probability that is missed.}



\section{Lower Bound}

\begin{theorem}
Let $\eps=O(1)$. Then any algorithm for estimating $s$-sparse distributions to within $\alpha$ in total variation requires at least 
\begin{align}
\Omega\Paren{\frac{s^2\log (k/s)}{\alpha^2(e^\eps-1)^2}}
\end{align}
samples.
\end{theorem}

We apply the chi-square contraction bounds to derive lower bounds for estimating sparse distributions. 

Consider a collection of ${k \choose s}$ distributions over $[k]\cup\{0\}$, each of which have $\p(0)=1-5\alpha$. For each $Z\in\{0,1\}^\ab$ with $s$ one's, the distribution $\p_Z$ has $\p_Z(i)=5\alpha/s$ if $Z_i=1$, and $\p_Z(i)=0$ otherwise. Now, fix any LDP channel $W$. Let $\q$ be the distribution with $\q(0)=1-5\alpha$, and $\q(i) = 5\alpha/k$ for other $i$'s. 

Therefore, the chi-squared distance between the output distrbutions for $\p_Z$ and $\p$ is
\begin{align}
\EE_{Z}[\chi^2(\p_Z^W,\p^W)] = \sum_y \frac{\EE_{Z}[\Paren{\sum_i (\p_Z(i)-\p(i)) W(y|i)}^2]}{\EE_{\p}[W(y|i)]}.
\end{align}

Then $\p_Z(i) -\p(i) = 5\alpha \Paren{\frac{-1}{\ab}+{\frac{Z_i}{s}}}$. Let $\bar{W}=\min_i W(y|i)$, and therefore, $W(y|i) = W_0^y +W_0(\eta^y_i)$, where $0<\eta^y_i \le e^{\eps}-1$.

\begin{align}
\sum_i (\p_Z(i)-\p(i)) W(y|i) &= 
5\alpha \sum_i \Paren{\frac{-1}{\ab}+Z_i{\frac{Z_i}{s}}}\Paren{W_0^y +W_0\eta^y_i}\\
& = 5\alpha W_0^y \sum_i \Paren{\frac{-1}{\ab}+{\frac{Z_i}{s}}}\eta^y_i.
\end{align}

Now, note that $\EE[Z_i]=\EE[Z_i^2]=s/k$, and $\EE[Z_iZ_j] = \frac{s(s-1)}{\ab(\ab-1)}$ for $i\ne j$. Therefore, 

\begin{align}
\EE_Z\left[\Paren{\sum_i (\p_Z(i)-\p(i)) W(y|i) }^2\right]
&= 25\alpha^2 (W_0^y )^2 \Paren{\sum_{i,j}\EE_Z\left[\frac 1{\ab^2} -\frac{Z_i+Z_j}{s\ab}+\frac{Z_iZ_j}{s^2}\right]\eta^y_i\eta^y_j}\\
&= 25\alpha^2 (W_0^y )^2 \Paren{\sum_{i}\left[\frac{1}{s\ab}-\frac 1{\ab^2}\right](\eta^y_i)^2+\sum_{i,j}\EE_Z\left[-\frac 1{\ab^2}+\frac{s-1}{s\ab(\ab-1)}\right]\eta^y_i\eta^y_j}\\
&\le 25\alpha^2 (W_0^y )^2 \Paren{\frac{(\max_i \eta^y_i)^2}{s}},
\end{align}
and 
\begin{align}
\frac{\EE_Z\left[\Paren{\sum_i (\p_Z(i)-\p(i)) W(y|i) }^2\right]}{\EE_{\p}[W(y|i)]} \le 25\alpha^2  \Paren{\frac{(\max_i \eta^y_i)^2}{s}}\cdot W_0^y 
\end{align}

Therefore, using $\sum_y W_0^y \le 1$, 
\begin{align}
\EE_{Z}[\chi^2(\p_Z^W,\p^W)] = O\Paren{\frac{\alpha^2 (e^\eps-1)^2}s}.
\end{align}


Now, note that within $\p_Z$ there exists a class of ${k\choose s/2}$ distributions that are at a distance $\alpha$ from each other. Therefore there is a packing with $\exp(s\log \frac ks)$ distributions, thus giving the proof. 

 








==> upper_LDP_old.tex <==
In this section, we analyze the sample complexity of sparse discrete distribution estimation under LDP constraints. We present two versions of Algorithm~\ref{alg:hadamard}, which are variants of the 1-bit Hadamard Response algorithm in~\cite{AcharyaS19}. Both variants are private-coin algorithms with only 1-bit communication from each user and run in $\tilde{O}(n+k)$ time. In Section~\ref{sec:ldp_upper_a}, we analyze Algorithm~\ref{alg:hadamard}(a), which is agnostic of the sparsity parameter $s$ and simply projects the output of 1-bit Hadamard Response algorithm in~\cite{AcharyaS19} onto $\Delta_k$. The algorithm achieves a sample complexity upper bound of $O(s^2 \log (k) /\alpha^2 \eps^2)$ as stated in Theorem~\ref{thm:ldp_sparse_b}, which is within a logrithmic factor of the optimal rate. The analysis is relatively straightforward but conveys the idea of why sparsity helps. In Section~\ref{sec:ldp_upper_b}, we analyze Algorithm~\ref{alg:hadamard}(b), which knows the sparsity parameter $s$ and achieves the optimal sample complexity of $O(s^2 \log (k/s) /\alpha^2 \eps^2)$ in Theorem~\ref{thm:ldp_sparse}. The analysis relies on a standard but more involved technique in sparse estimation based on a covering set argument.


To establish the optimality of the sample complexity bounds in Theorem~\ref{thm:ldp_sparse}, we design a family of $s$-sparse distributions and show that it is hard to estimate the distribution within the family. The techniques involve a variant of Fano's inequality in~\cite{duchi2013distance} and $\chi^2$-contraction bounds developed recently in~\cite{AcharyaCT19}. Details are presented in Section~\ref{sec:ldp_lower}.

\begin{algorithm2e}[h]
	\caption{1-bit Hadamard Response with Projection}
	\label{alg:hadamard}
	\KwIn{$X_1, \ldots, X_n$ i.i.d. from $p\in\Delta_{k, s}$, (For version (b), the sparsity parameter $s$). }
	\KwOut{$\hp\in\Delta_k:$ an estimate of $p$}
	$K=2^{\lceil\log_2(k+1) \rceil}$. Let $H_K$ be the $K$-dimensional Hadamard matrix defined in Definition~\ref{def:hadamard}.
	
	For $y \in[K]$, 
	\[ B_y:=\{x\in[K]:H_{K}(x, y)=1\}. \] \\
	Divide $n$ users into $K$ sets. $\forall j \in [K]$, 
	\[ S_j :=\{i \in [n]: j \equiv i \mod K \}.\] 
	
	For user $i$, let $j_i\in [K]$ be such that $ i \equiv j_i \mod K$, and  
	\begin{align*}
		\label{equ:scheme}
		\Pr(Y_i=1)=\begin{cases}
			\frac{e^\eps}{e^\eps + 1}, &X_i\in B_{j_i},\\
			\frac{1}{e^\eps + 1},&\text{otherwise}.
		\end{cases}
	\end{align*}
	
	Let $\hat{s}:=(\hat{s}_1, \ldots, \hat{s}_{K})$ where $\forall j \in [K]$,
	\[
		\hat{s}_j :=\frac{1}{|S_j|}\sum_{i\in S_j}Y_i.
	\] 
	
	
	Compute intermediate estimates for 
	\[ 
		\tp_K:=\frac{e^\eps+1}{K (e^\eps - 1)} H_K (2\hat{s}-\mathbf{1}_K).
	\] \label{step:before_projection} 
	
	Keep the first $k$ elements in $\tp_K$, i.e. $\tp:=\tp_K^{[k]}$ and project it onto $\Theta$ (For version (a), $\Theta = \Delta_k$ and for version (b), $\Theta = \setsp$), 
	\[
		\hp := \min_{\p \in \Theta} \norm{\tp - \p}{2}^2.
	\] \label{step:projection}
\end{algorithm2e}



\subsection{Sparse Estimation Without Knowing $s$} \label{sec:ldp_upper_a}

In this section, we analyze the performance of Algorithm~\ref{alg:hadamard}(a) and prove the upper bound part of Theorem~\ref{thm:ldp_sparse_b}. Before proceeding to prove the performance, we note here that both versions of Algorithm~\ref{alg:hadamard} can be implemented in $\tilde{O}(n+k)$ time, which is almost linear in the size of the input. By~\cite{AcharyaS19}, we can obtain $\tilde{p}$ in Step~\ref{step:before_projection} in Algorithm~\ref{alg:hadamard}(a) in $\tilde{O}(n+k)$ time. By~\cite{duchi2008efficient} and~\cite[Algorithm 1]{kyrillidis2013sparse}, Step~\ref{step:projection} can also be implemented in $\tilde{O}(k)$ time, proving the overall time complexity.
We first present the definition of Hadamard matrices and state one of their well-known properties.
\begin{definition}
	\label{def:hadamard}
	Let $H_1:=[1]$. For $m=2^j, j\ge 1$, recursively define $H_m$ as:
	\[
	H_m:=\begin{bmatrix}
	H_{m/2} & H_{m/2}\\
	H_{m/2} & -H_{m/2}
	\end{bmatrix}.
	\]
\end{definition}
We will use the following well-known property of Hadamard matrices.
\begin{claim}
	\label{clm:hadamard}
	The Hadamard matrix $H_K$  defined in Definition \ref{def:hadamard} satisfies
	\[
	H_K^T H_K = K I_K.
	\]
\end{claim}



The privacy guarantee follows from~\cite{AcharyaS19}. %
The proof mainly focuses on analyzing the projection step (Step~\ref{step:projection}). %
By the definiton of $\hp$, we have $\norm{\tp - \hp}{2}^2 \le \norm{\tp - \p}{2}^2$. Hence
\[
\norm{\tp - \p}{2}^2 \ge \norm{\tp - \hp}{2}^2 = \norm{\tp - \p}{2}^2 + \norm{\p - \hp}{2}^2  + 2 \langle\tp - \p, \p - \hp\rangle.
\]

Rearranging the terms we have,
\begin{equation} \label{eqn:key_inequality}
\norm{\p - \hp}{2}^2 \le 2 \langle\tp - \p, \hp - \p\rangle.
\end{equation}

By Holder's inequality, we get
\begin{equation} \label{eqn:infty_l1}
\norm{\p - \hp}{2}^2 \le 2 \langle\tp - \p, \hp - \p\rangle \le 2 \norm{\tp - \p}{\infty} \norm{\hp - \p}{1}. \nonumber 
\end{equation}

Next, suppose $\p$ is supported over $S$ where $|S| \le s$.
\begin{equation}
\label{eqn:l1_l2}
\norm{\hp - \p}{1} = \norm{\hp^{S} - \p^{S}}{1} +  \norm{\hp^{S^c} - \p^{S^c}}{1}  \le 2 \norm{\hp^{S} - \p^{S}}{1} \le 2 \sqrt{s} \norm{\hp^{S} - \p^{S}}{2} \le 2 \sqrt{s} \norm{\hp - \p}{2}. 
\end{equation}

Hence
\begin{equation}
\label{eqn:l2_upper}
\norm{\p - \hp}{2}\le 2\sqrt{s}\norm{\tp - \p}{\infty}.
\end{equation}


Let $e_x$ be the standard basis vector at dimension $x$. From~\cite{AcharyaS19}, we have $\langle \tp - \p, e_j \rangle$ is zero-mean and sub-Gaussian with variance proxy at most
\[
	\frac{2}{n}\left(\frac{e^\eps+1}{e^\eps-1}\right)^2.
\]
Thus by the maximal inequalities of sub-Gaussian random variables~\cite{rigollet2015high}, with probability at least $9/10$, we have:
\begin{equation} \label{eqn:infty_bound}
\norm{\tp - \p}{\infty}\le \frac{3(e^\eps + 1)\sqrt{\log (2k)}}{(e^\eps -1 )\sqrt{n}}. \nonumber 
\end{equation}

Combining with~\eqref{eqn:l1_l2} and~\eqref{eqn:l2_upper} and setting the right hand side to be $\alpha$ yields the desired bound.

\subsection{Optimal Upper Bound for Sparse Discrete Distribution Estimation} \label{sec:ldp_upper_b}
In this section, we analyze the performance of Algorithm~\ref{alg:hadamard}(b) and prove the upper bound part of Theorem~\ref{thm:ldp_sparse}. The analysis borrows ideas from~\cite{raskutti2011minimax} for high-dimensional sparse regression.  %





	
	
	We will use the following bound on the covering number of $s$-sparse vectors. 
	\begin{claim}[\cite{raskutti2011minimax}]
		Let $S(r, 2s) = \{ \err \in \RR^k:  \norm{\err}{2} \le r,  \norm{\err}{0} \le 2s\}$. There exists a $\rho r$-covering $\cC_r \subset S(r, 2s)$ of $S(r, 2s)$ with size
		\[
			|\cC_r|=N(S(r, 2s), \rho r) \le {k \choose 2s} \Paren{\frac{1}{\rho}}^{2s}.
		\]
	\end{claim}
	
	
	Let $\cC_1$ be a $\rho$-covering of $S(1, 2s)$ with size $N(S(1, 2r), \rho)$. Let $r = \norm{\hp - p}{2}$, then $\hp - p \in S(r, 2s)$, and one can obtain a covering $\cC_r$ of $S(r, 2s)$ by multiplying each vector in $\cC_1$ by $r$. 
	
	Since $\hp - p$ is $2s$-sparse, let $\err^*$ be the closest point in $\cC_r$ to $\hp - p$. Then we can bound the right hand side of~\eqref{eqn:key_inequality}.
	\begin{align*}
		\langle \tp - \p, \hp - \p\rangle & \le |\langle\tp - \p, \err^* \rangle| + |\langle\tp - \p, \hp - \p - \err^* \rangle| \\
		& \le \max_{\err \in \cC_r}|\langle \tp - \p, \err \rangle| + \rho r \norm{\tp - \p}{2} \\
		& = r\max_{\err \in \cC_r}|\langle \tp - \p, \err/r \rangle| + \rho r \norm{\tp - \p}{2} \\
		& = r\max_{\err \in \cC_1}|\langle \tp - \p, \err \rangle| + \rho r \norm{\tp - \p}{2}.
	\end{align*}
	
	Let $s:=(s_1, \ldots, s_{K})$ where $\forall j \in [K]$,
	\[
		s_j = \probof{Y_i = 1 \mid i \in S_j}.
	\] 
	Then we have $\expectation{\hat{s}} = s$. Note that in Algorithm~\ref{alg:hadamard}, 	$\forall j \in [K]$, $\hat{s}_j$ is the average of $|S_j| \ge K/(2n)$ i.i.d Bernoulli random variables. Hence $\forall i \in [K], \hat{s}_j- s_j$ is a zero-mean sub-Gaussian random variable with variance proxy at most $\frac{K}{n}$. Moreover, $\hat{s}_j$'s are independent since $S_j$'s are disjoint. Let $p_K$ be a distribution over $[K]$ obtained by appending zeros to $p$. From~\cite{AcharyaS19}, we have
	\[
		\tp_K - \p_K = \frac{2(e^\eps+1)}{K (e^\eps - 1)} H_K (\hat{s}-s).
	\]
	Hence for all $\forall \err\in \cC_1$, 
	\[
		\langle \tp_K - \p_K, \err\rangle = \frac{2(e^\eps+1)}{K (e^\eps - 1)}  \err^T H_K (\hat{s}-s),
	\]
	which is a linear combination of $(\hat{s}_j - s_j)$'s, which are independent sub-Gaussian random variables. Since $\tp - \p$ is the first $k$ entries of $\tp_K - \p_K$, we have $\forall e \in \cC_1$, $\langle \tp - \p, \err \rangle$ is also sub-Gaussian (see Corollary 1.7 in~\cite{rigollet2015high}) with variance proxy at most
	\[
	\frac{K}{2n} \left\|\frac{2(e^\eps+1)}{K (e^\eps - 1)}  \err^T H_K\right\|_2^2 = \frac{2}{n K} \Paren{\frac{e^\eps+1}{e^\eps-1}}^2    \left \|\err^T H_K\right\|_2^2 = \frac{2}{n} \Paren{\frac{e^\eps+1}{e^\eps-1}}^2    \left \|\err\right\|_2^2 \le \frac{2}{n}\left(\frac{e^\eps+1}{e^\eps-1}\right)^2 =:\sigma^2.
	\]
	
	
	
	Therefore using maximal inequalties of sub-Gaussian random variables~\cite[Theorem 1.14]{rigollet2015high}, with probability at least $19/20$, we have 
	\[
		\max_{e \in \cC_1}|\langle \tp - \p, \err \rangle| < \sigma \sqrt{14\log|\cC_1|}.
	\]
	Furthermore, by the utility guarantee of Hadamard Response~\cite{AcharyaS19}, with probability at least $19/20$, 
	\[
	\|\tp- p\|_2^2\le 20\EE[\|\tp- p\|_2^2]\le \frac{40k(e^\eps+1)^2}{n(e^\eps-1)^2}\implies \|\tp- p\|_2 \le 7\frac{e^\eps +1 }{e^\eps -1 }\sqrt{\frac{k}{n}}.
	\]
	By union bound, conditioned on these two evenets, which happens with probability at least $9/10$,
	\begin{align*}
		\langle \tp - \p, \hp - \p\rangle &\le \frac{e^\eps+1}{e^\eps-1}\frac{r}{\sqrt{n}} \sqrt{56\log |\cC_1|} + 7\rho r \frac{e^\eps+1}{e^\eps-1}\sqrt{\frac{k}{n}}  \\
		& \le \frac{e^\eps+1}{e^\eps-1}\frac{r}{\sqrt{n}} \sqrt{112s \log\left(\frac{ek}{2s}\right) + 112s \log \frac{1}{\rho}}  +7\rho r \frac{e^\eps+1}{e^\eps-1}\sqrt{\frac{k}{n}}.
	\end{align*}
	Taking $\rho = \sqrt{\frac{s}{k}}$, 
	\[
	\langle \tp - \p, \hp - \p\rangle \le 25\frac{e^\eps+1}{e^\eps-1}\frac{r \sqrt{s\log(2k/s)} }{\sqrt{n}} = 25\frac{e^\eps+1}{e^\eps-1}\frac{\sqrt{s \log(2k/s)} }{\sqrt{n}} \norm{\hp - p}{2}.
	\]
	Combining with~\eqref{eqn:key_inequality}, 
	\[
	\norm{\hp - p}{2} \le \frac{25(e^\eps+1) \sqrt{s\log(2k/s)} }{(e^\eps-1)\sqrt{n}}.
	\]
	Since $\hp - p$ is $2s$-sparse, by Cauchy-Schwartz,
	\[
	d_{TV}(\hp, \p)=\frac{1}{2}\norm{\hp - p}{1} \le \frac{1}{2}\sqrt{2s}\norm{\hp - p}{2} \le \frac{20s \sqrt{\log(2k/s)}}{\sqrt{n}}\frac{e^\eps+1}{e^\eps-1}.
	\]
	Setting the right hand side as $\alpha$ yields the desired sample complexity bound.
	



    












==> upper_communication.tex <==
We now prove the results for communication constrained sparse discrete distribution estimation. In Section~\ref{sec:lbit_upper}, we propose a public-coin SMP protocol and prove that its  sample complexity is $O(s^2\log(\ab/s)/(\alpha^2\min\{s, 2^\ell\}))$, the upper bound of Theorem~\ref{thm:lbit_sparse}. Our lower bounds of Theorem~\ref{thm:lbit_sparse} are shown in Section~\ref{sec:lbit_lower}.

\subsection{$\ell$-bit communication upper bound} \label{sec:lbit_upper}

We first present our scheme, where we use public randomness to design hash functions at the users. 
\begin{definition}
	A randomized mapping $h: [\ab] \rightarrow [2^{\ell}]$ is a random hash function if
	\[
		x \in[\ab], y \in [2^\ell], \quad  \probof{h(x) = y} = \frac{1}{2^{\ell}}.
	\]
\end{definition}

\noindent\textbf{The scheme.} We assume $\ns$ independent hash functions $h_1, \ldots, h_\ns$ are available at the users, which can be achieved using the public randomness. User $i$ outputs $Y_i=h_i(X_i)$. Therefore, the channel of user $i$ is $W_i=h_i$, with an $\ell$ bit output. 

\noindent\textbf{The estimator.} Upon receiving messages $Y_1,\ldots, Y_\ns$, the estimator is as follows. 
\begin{enumerate}
	\item
	We use the messages from the first $\nsein$ users to obtain a subset $T\subseteq[k]$ with $|T|=O(s)$ such that with high probability $p(T)>1-\alpha/25$.  
	\item 
	 With the remaining messages we estimate $p(x)$ for $x\in T$. 
\end{enumerate}

We now describe and analyze the two steps. 

\noindent\textbf{Step 1.} Let $Y_1, \ldots, Y_{\nsein}$ be the first $n/2$ messages, where $Y_i = h_i(X_i)$. For $x=1,\ldots, \ab$, let $\ms(x):=|\{i:h_i(x)=Y_i, 1\le i \le \nsein\}|$ be the number of these messages such that $x$ belongs to the preimage of $Y_i$. Let $T\subseteq [\ab]$ be the set consisting of the largest $|T|=\min\{2s, \ab\}$ values of $\ms(x)$'s. If $\p(x)$ is large then we expect $\ms(x)$ to be large. We formalize this and  show that for sufficiently large $n$, the probability of symbols not in $T$  is small.
\begin{lemma}
\label{lem:step-one}
There is a constant $C$ such that for $n= C\cdot{s^2\log (\ab/s)}/({\alpha^2 \min\{2^\ell,s\}})$ with probability at least $0.99$, $p(T)>1-\alpha/25$.
\end{lemma}

\noindent\textbf{Step 2.}  For $x=1,\ldots, \ab$, let $N(x):=|\{i:h_i(x)=Y_i, \nsein<i\le \ns \}|$ be the number of messages  in the second half such that $x$ belongs to the preimage of $Y_i$. Our estimator is given by
\begin{equation}\label{eqn:phat-comm}
\hat p(x) = \begin{cases}
	\frac{(2^\ell N(x)/(\nsein))-1}{2^\ell-1},& \text{if $x\in T$}\\
	0, &\text{otherwise.}
\end{cases}
\end{equation}

We now show that $\hat p$ converges to $p$ over $T$. 
\begin{theorem}
	\label{thm:utility_com}
	\[
		\expectation{\norm{\hp^T - p^T}{1}}\le \sqrt{\frac{16s^2 2^\ell }{\ns(2^\ell-1)^2}}.
	\]
\end{theorem}

Combining Theorem~\ref{thm:utility_com} and Lemma~\ref{lem:step-one} gives the upper bound of Theorem~\ref{thm:lbit_sparse} with an application of Markov's inequality. 

We now prove Theorem~\ref{thm:utility_com} and Lemma~\ref{lem:step-one}. The observation here is that for any $i$ and $x\in[\ab]$, 
\begin{align}\label{eqn:pre-image}
 	\bias(x):= \probof{Y_i = h_i(x)}= \p(x)+(1-\p(x))\frac1{2^\ell} = \p(x)\left(1-\frac{1}{2^\ell}\right)+\frac{1}{2^\ell}.
 \end{align}





\begin{proof}[Proof of Theorem~\ref{thm:utility_com}]
$N(x)$ is distributed as a Binomial ${Bin}(\ns/2,\bias(x))$. Hence, $\expectation{N(x)}=\ns \cdot \bias(x)/2$. By~\eqref{eqn:pre-image} and~\eqref{eqn:phat-comm} we have $\expectation{\hp(x)}=\p(x)$. Using the variance formula of Binomials, we know $\variance{N(x)}=\ns\cdot \bias(x)\cdot(1-\bias(x))/2\le \ns\cdot \bias(x)/2$.
\begin{align}
\expectation{(\hp(x)-p(x))^2} = \left(\frac{2\cdot2^\ell}{\ns(2^\ell-1)}\right)^2,\; \variance{N(x)} \le \frac{2}{\ns}\left(\frac{2^\ell}{2^\ell-1}\right)^2 \bias(x).
\end{align}
Now, note that $\sum_{x\in T} \bias(x) = p(T)(1-1/2^\ell)+|T|/2^\ell$, and therefore,

\begin{align*}
\expectation{\norm{\hp^T-p^T}{2}^2} = \sum_{x\in T}\expectation{(\hp(x)-p(x))^2}%
\le \frac{2}{\ns}\left(\frac{2^\ell}{2^\ell-1}\right)^2\sum_{x\in T} \bias(x)
\le \frac{4|T|2^\ell}{\ns (2^\ell-1)^2}.
\end{align*}
Theorem~\ref{thm:utility_com} now follows by using Jensen's inequality and Cauchy Schwarz:
\[
\left(\expectation{\norm{\hp^T - \p^T}{1}}\right)^2\le \expectation{\norm{\hp^T - \p^T}{1}^2}\le |T|\cdot\expectation{\norm{\hp^T - \p^T}{2}^2}.
\]
\end{proof}
\begin{proof}[Upper bound of Lemma~\ref{lem:step-one}]
Note that $\ms(x)$ and $N(x)$ are identically distributed, and therefore,  $\ms(x)$ is Binomial ${Bin}(\ns/2,\bias(x))$. Hence, $\expectation{\ms(x)}=\ns \cdot b(x)/2$.

Set $\gamma=1-1/2^\ell$ and $\beta=1/2^\ell$, then $\bias(x)= \gamma\cdot p(x)+\beta$. We will use the multiplicative Chernoff bound (Lemma~\ref{lem:chernoff}).
\begin{lemma}[Multiplicative Chernoff bound] \label{lem:chernoff}
Let $Y_1, \ldots, Y_n$ be independent random variables with $Y_i\in[-1,1]$, and $Y = Y_1+\dots+Y_\ns$, and $\mu= \expectation{Y}$. Then for $\tau>0$, 
\begin{align*}
    \probof{Y>(1+\tau)\mu}<e^{-\frac{\tau^2\mu}{2+\tau}},\quad    \probof{Y<(1-\tau)\mu}<e^{-\frac{\tau^2\mu}{2}}.
\end{align*}
\end{lemma}

Let $S$ be the set of elements with non-zero probability. If $x \in [\ab]\setminus S$, then $p(x)=0$. Hence by Lemma~\ref{lem:chernoff},
\[
\probof{\ms(x)\ge \nse\beta +C_1\sqrt{\nse \beta\log \frac \ab s}}\le \Paren{\frac s\ab}^{C_1^2/2}.
\]

Let $E$ be the event that at most $s$ symbols in $[\ab]\setminus S$ appear more than $\ms^\ast :=\nse\beta +C_1\sqrt{\nse \beta \log \frac ks}$ times. By Markov's inequality,
\begin{align*}
\probof{E^c}=\probof{\left|x \in [\ab]\setminus S: \ms(x)\ge \nse\beta +C_1\sqrt{\nse \beta \log \frac \ab s}\right|>s}\le \Paren{\frac s\ab}^{C_1^2/2-1}.
\end{align*}


We condition on the event $E$ for the remaining part of the proof. We claim that for $n$ appropriately chosen, the set $T$ contains most of the probability density, formally stated in Lemma \ref{lem:step-one}.


Conditioned on $E$, a symbol $x$ is not selected after the first stage only if it appears at most  $\ms^\ast$ times, which implies $\condprob{x \text{ not selected}}{E}\le \condprob{\ms(x)<\ms^\ast}{E}$. 
Moreover, since $\forall x_1 \in S, x_2 \notin S$, $\ms(x_1)$ and $\ms(x_2)$ are independent, we have $\ms(x_1)$ is independent of event $E$. Thus:


\begin{align*}
\condexpect{\p(T^c)}{E} &=\sum_x\p(x)\condprob{x \text{ not selected}}{E}\le 
\sum_x\p(x)\condprob{\ms(x)<\ms^\ast}{E}\\
&\le \sum_{x:\p(x)>\alpha/50s}\p(i)\condprob{\ms(x)<\ms^\ast}{E}+\frac{\alpha}{50}\\
& = \sum_{x:\p(x)>\alpha/50s}\p(i)\probof{\ms(x)<\ms^\ast}+\frac{\alpha}{50}.
\end{align*}

It is sufficient to bound the sum by $\alpha/50$. To prove that, we consider two cases separately: $\p(x)\le C\beta/\gamma$ and $\p(x)>C\beta/\gamma$ where $C=2e-1$. Define $U:=\{x\in[\ab]:\p(x)>\alpha/50 s\}$ and $I:=\{x\in U: \p(x)\le C\beta/\gamma\}$.

\paragraph{Case 1.} $\p(x) \le C \beta/\gamma$. In this case,
\begin{align*}
\expectation{\ms(x)-\ms^\ast}=\nse \gamma\p(x)-C_1\sqrt{\nse \beta \log \frac \ab s},
\end{align*}
and for $\nse = 1250 C_1^2 \beta\frac{s^2\log \frac \ab s}{\alpha^2\gamma^2}$, using $\p(x)>\alpha/50s$,
\begin{align*}
\frac12 \nse \gamma\p(x)-C_1\sqrt{\nse \beta \log \frac \ab s}\ge 0,
\end{align*}
which implies
$
\expectation{\ms(x)-\ms^\ast}\ge\nse \p(x)/(2\gamma).
$
Using Lemma~\ref{lem:chernoff},
\begin{align*}
\probof{\ms(x) \le \ms^\ast} 
&= \probof{\ms(x) \le \expectation{\ms(x)} -(\expectation{\ms(x)} -\ms^\ast)}\\
&\le \exp\Paren{-(\frac{\gamma p(x)/2}{\gamma p(x)+ \beta})^2 \nse (\gamma p(x) + \beta)}\\
& = \exp\Paren{-\frac{\gamma^2 p(x)^2\nse}{4(\gamma p(x) + \beta)} } \\
& \le \max \left\{\exp\Paren{-\frac{\gamma^2 p(x)^2\nse}{8\beta} }, \exp\Paren{-\frac{\gamma p(x)\nse}{8} } \right\}.
\end{align*}
Since $p(x) \le C \beta/\gamma$,
\[
    \probof{\ms(x) \le \ms^\ast} \le \exp\Paren{-\frac{\gamma^2 p(x)^2\nse}{8C\beta} }.
\]
Now for $\p(x)=(1+\zeta_x)\alpha/50s$ where $\zeta_x>0$, we have 
\begin{align*}
\frac{\gamma^2 p(x)^2\nse}{8C\beta} \ge 125 C_1^2/C(1+\zeta_x)^2 \log \frac \ab s,
\end{align*}
and therefore, 
\begin{align*}
\sum_{x\in I}p(x)\probof{\ms(x) \le \ms^*} \le 
\frac \alpha{50s}\sum_{x\in I} (1+\zeta_x)\exp\Paren{-125C_1^2/C (1+\zeta_x)^2\log \frac \ab s}\le \frac {\alpha}{100}.
\end{align*}

\paragraph{Case 2:} $p(x)> C\beta/\gamma$. We first consider the case when $p(x) \le 1/2$.
\begin{align*}
    \probof{\ms(x) \le \ms^\ast}  & = \sum_{t = 0}^{\floor{\ms^\ast}} {\nse \choose t} (\gamma p(x) + \beta)^t (1 - \gamma p(x) - \beta)^{\nse - t}.
\end{align*}

Moreover, since $\ms^\ast =\nse\beta +C_1\sqrt{\nse \beta \log \frac\ab s} \le n\beta$,
\begin{align*}
    \probof{\ms(x) \le \ms^\ast}  & \le \ns \beta {\nse \choose \ns\beta}(\gamma p(x) + \beta)^{\ns\beta} (1 - \gamma p(x) - \beta)^{\nse - \ns\beta}\\
    & \le n \beta \Paren{\frac{e \nse}{\ns\beta}}^{\ns \beta}(\gamma p(x) + \beta)^{\ns\beta } (1 - \gamma p(x) - \beta)^{\nse - n\beta } \\
    & \le \ns \beta  \Paren{\frac{e (\gamma p(x)+ \beta)}{2\beta (1 - \gamma p(x)- \beta)}}^{\ns \beta} \Paren{(1 - \gamma p(x) - \beta)^{\frac{1}{2\beta}}}^{\ns \beta}\\
    & \le \ns\beta  \Paren{\frac{e (\gamma p(x) + \beta)}{\beta }}^{\ns \beta} \Paren{e^{-\frac{\gamma p(x) + \beta}{2 \beta}}}^{\ns \beta} \\
    & = \ns\beta  \Paren{\frac{e (\gamma p(x) + \beta)}{\beta } e^{-\frac{\gamma p(x)+ \beta}{2 \beta}}}^{\ns \beta}. 
\end{align*}
Using $2e t e^{-t} \le \frac{1}{t} $ when $t \ge 2$ and $\gamma p(x) + \beta > 2e\beta$, 
\begin{align*}
    \probof{\ms(x) \le \ms^\ast} & \le 2\nse\beta  \Paren{\frac{e (\gamma p(x) + \beta)}{\beta } e^{-\frac{\gamma p(x) + \beta}{2 \beta}}}^{2\nse \beta} \le 2\nse\beta \Paren{\frac{\gamma p(x) + \beta}{2 \beta}}^{-2\nse\beta }  \\
    & \le 2\nse\beta e^{-2\nse\beta } \le \frac{1}{2\nse\beta} \le \frac{\alpha}{100}.
\end{align*}
When $\p(x) > 1/2$, the probability will not be higher than this. Hence, 
\[
\sum_{x \in U\setminus I}p(x)\probof{\ms(x)\le \ms^*}  \le \frac{\alpha}{100}.
\]

Combining the two cases we have,
\begin{align*}
\sum_{x :\p(x)>\alpha/50s}\p(x)\probof{\ms(x)\le \ms^*}&=\sum_{x\in I}\p(x)\probof{\ms(x)\le \ms^*} + \sum_{x\in U \setminus I}p(x)\probof{\ms(x)\le \ms^*}  \le  \frac{\alpha }{50}.
\end{align*}

In the second stage, by Theorem \ref{thm:utility_com}, with $\nse$ samples we can guarantee that
\[
	\condexpect{\sum_{x\in T}|\hp(x)-p(x)|}{E}\le \frac{\alpha}{25}.
\]
Hence, conditioned on $E$,
\[
    \condexpect{\norm{\hp-\p}{1}}{E}=\condexpect{\sum_{x\in T}|\hp(x)-p(x)|}{E}+\condexpect{p(T^c)}{E}\le \frac{2}{25}\alpha < \frac{1}{10}\alpha.
\]
Finally by Markov's inequality, conditioned on $E$ with probability at least $19/20$, 
\[
    d_{TV}(\hp, \p)\le \frac{1}{2}\norm{\hp - \p}{1}\le \alpha.
\]
Together the above accuracy is guaranteed with probability at least 1/10. Finally, note that the number of samples
\[
	\ns=2500C_1^2 \beta \frac{s^2\log \frac \ab s}{\alpha^2\gamma^2} =2500 C_1^2\frac{s^22^\ell\log\frac \ab s}{\alpha^2(2^\ell -1)^2},
\]
which yields the desired sample complexity.


\end{proof}



















